Accelerating Chance-constrained SCED via Scenario Compression

This paper studies some compression methods to accelerate the scenario-based chance-constrained security-constrained economic dispatch (SCED) problem. In particular, we show that by exclusively employing the vertices after convex hull compression, an equivalent solution can be obtained compared to utilizing the entire scenario set. For other compression methods that might relax the original solution, such as box compression, this paper presents the compression risk validation scheme to assess the risk arising from the sample space. By quantifying the risk associated with compression, decision-makers are empowered to select either solution risk or compression risk as the risk metric, depending on the complexity of specific problems. Numerical examples based on the 118-bus system and synthetic Texas grids compare these two risk metrics. The results also demonstrate the efficiency of compression methods in both problem formulation and solving processes.

==> Another_Method.tex <==
\section{Method 1}
\indent Step 1: Construct a convex hull $\mathcal{H}$ generated from scenarios $\tilde{w}_i \quad i=1,2,3,...,N$ and express $\mathcal{H}$ by the polyhedron:
\begin{equation} \label{polyhedron}
A\tilde{w} \leq b
\end{equation}
\indent Step 2: Relax the scenario-based problem to the robust optimization problem under polyhedron uncertainty where each inequality constraint in (\ref{subeqn:risk}) can be replaced by robust form. Take $f(\hat{w}, \tilde{w}) \preceq \bar{f}$ for example:
\begin{equation} \label{max}
\max _{\tilde{w}}\; f(\hat{w}, \tilde{w})_j \leq \bar{f}_j \quad j=1,2,...,l
\end{equation}
where $l$ is the number of lines in the network.\\
\indent The above min-max two stages problem is even harder to solve efficiently than the previous scenario-based problem, but we can convert it to a min-min version by dual analysis and combine the two minimization problems together.\\
\indent Step 3: Take the dual of the inner optimization problem in (\ref{max}). More detail is shown in (\ref{lagradetail}).\\
\begin{equation} \label{lagral}
\begin{aligned}
\min _{\lambda}\; &-\lambda^{\top}b -(H_d d)_j+(H_w \hat{w})_j+(H_g g)_j \\
s.t. & \quad \lambda^{\top}A + (H_w)_j-(H_g\eta\mathbf{1}^{\top})_j =0\\
& \quad \lambda \succeq 0
\end{aligned}
\end{equation}
\indent Step 4: Combine min-min problems together. Take (\ref{lagral}) for example:
\begin{equation} \label{combine}
\begin{aligned}
\min _{g, \eta, \lambda}\; &c(g)\\
s.t. &-\lambda^{\top}b -(H_d d)_j+(H_w \hat{w})_j+(H_g g)_j \leq \bar{f}_j\\
& \quad \lambda^{\top}A + (H_w)_j-(H_g\eta\mathbf{1}^{\top})_j =0 \quad j=1,2,...,l\\
& \quad \lambda \succeq 0
\end{aligned}
\end{equation}

\begin{strip}
\begin{align}\label{lagradetail}
L(\tilde{w},\lambda)&=(H_w)_j\tilde{w}-(H_g\eta\mathbf{1}^{\top})_j \tilde{w}-(H_d d)_j+(H_w \hat{w})_j+(H_g g)_j+\lambda^{\top}(A\tilde{w}-b)\\
&=\{(H_w)_j-(H_g\eta\mathbf{1}^{\top})_j+\lambda^{\top}A\} \tilde{w} -(H_d d)_j+(H_w \hat{w})_j+(H_g g)_j-\lambda^{\top}b\\
\sup _{\tilde{w}} L(\tilde{w},\lambda)& = -\lambda^{\top}b -(H_d d)_j+(H_w \hat{w})_j+(H_g g)_j \\
& \text{when} \quad \lambda^{\top}A + (H_w)_j-(H_g\eta\mathbf{1}^{\top})_j =0
\end{align}
\end{strip}

==> old.tex <==
\begin{definition}[Helly's Dimension]
Helly's dimension of the scenario problem $\mathrm{SP}(\mathcal{N})$ is the smallest integer $h$ that $h\geq_{\text{ess sup}\mathcal{N}\subseteq\Delta^N}|\mathcal{S(N)}|$ holds for any finite $N\geq1$, where $|\mathcal{S(N)}|$ is the number of support constraints or sample complexity.    
\end{definition}
\textit{Remark}: Because of the \textit{i.i.d.} sampled scenario, the solution complexity $|\mathcal{S(N)}|$ may change with each experiment, and the Helly's dimension is the upper bound of $|\mathcal{S(N)}|$. In practical application, when the uncertain variables have relatively simple distribution and $N$ is large, we directly use the $|\mathcal{S(N)}|$ of a given set of scenarios to approximate $h$ \cite{campi2018wait,modarresi2018scenario}.

Under the assumptions of non-degeneracy and feasibility of the optimization problem, the deepest results show that the distribution of $\mathbb{V}_{\tilde{w}}(g^*,\eta^*)$ is dominated by a Beta distribution, namely:
\begin{equation}
\label{ExactSP}
\mathbb{P}_{\tilde{w}}^N\left(\mathbb{V}_{\tilde{w}}(g^*,\eta^*)>\epsilon\right) \leq \sum_{i=0}^{h-1}\left(\begin{array}{c}
N \\
i
\end{array}\right) \epsilon^i(1-\epsilon)^{N-i} := \beta
\end{equation}
where $h$ is the Helly's dimension of $\mathrm{SP}(\mathcal{N})$, and $1-\beta$ is defined as the confidence bound for the solution based on any $N$ \textit{i.i.d} scenarios.\\


\section{Appendix}
\subsection{Calculation of $\underline{\varepsilon}_{k}$, $\bar{\varepsilon}_{k}$}
Construct the following function $\Psi_{k, \beta}:(-\infty, 1) \rightarrow \mathbb{R}$ indexed by $k=0,1,\dots,N$ and by the confidence parameter $\beta \in (0,1)$:\\
for $k=0,1,\dots,N-1$, let
\begin{equation}
\begin{aligned}
\Psi_{k, \beta}(\alpha)&=\frac{\beta}{2 N} \sum_{t=k}^{N-1} \frac{\left(\begin{array}{l}t \\ k\end{array}\right)}{\left(\begin{array}{l}N \\ k\end{array}\right)}(1-\alpha)^{-(N-t)} \\
&+\frac{\beta}{6 N} \sum_{t=N+1}^{4 N} \frac{\left(\begin{array}{c}t \\ k\end{array}\right)}{\left(\begin{array}{c}N \\ k\end{array}\right)}(1-\alpha)^{t-N}
\end{aligned}
\end{equation}
when $k=N$, let
\begin{equation}
\begin{aligned}
\Psi_{k, \beta}(\alpha)=\frac{\beta}{6 N} \sum_{t=N+1}^{4 N} \frac{\left(\begin{array}{c}t \\ k\end{array}\right)}{\left(\begin{array}{c}N \\ k\end{array}\right)}(1-\alpha)^{t-N}
\end{aligned}
\end{equation}
\indent It is shown in \cite{campi2023compression} that equation $\Psi_{k, \beta}(\alpha)=1$ admits only two solutions in $(-\infty,0)$ when $k=0,1,\dots,N-1$, denoting as $\underline{\alpha}_k$ and $\bar{\alpha}_k$, while only one solution when $k=N$, called $\underline{\alpha}_N$.\\
\indent Based on the above notations, the closed form of $\underline{\varepsilon}_{k}$ and $\bar{\varepsilon}_{k}$ can be expressed as 
\begin{equation} \label{lbound}
    \underline{\varepsilon}_k=\max \left\{0, \underline{\alpha}_k\right\}, \quad k=0,1, \ldots, N
\end{equation}
and
\begin{equation} \label{ubound}
    \bar{\varepsilon}_k= \begin{cases}\bar{\alpha}_k, & k=0,1, \ldots, N-1 \\ 1, & k=N\end{cases}
\end{equation}

\subsection{Simple Example}
